Dynamical scoto-seesaw mechanism with gauged $B-L$

We propose a dynamical scoto-seesaw mechanism using a gauged $B-L$ symmetry. Dark matter is reconciled with neutrino mass generation, in such a way that the atmospheric scale arises \textit{a la seesaw}, while the solar scale is \textit{scotogenic}, arising radiatively from the exchange of ``dark'' states. This way we ``explain'' the solar-to-atmospheric scale ratio. The TeV-scale seesaw mediator and the two dark fermions carry different $B-L$ charges. Dark matter stability follows from the residual matter parity that survives $B-L$ breaking. Besides having collider tests, the model implies sizeable charged lepton flavour violating (cLFV) phenomena, including Goldstone boson emission processes.

==> Makefile <==
FILENAME=GaugedScotoSeesaw-v2
LATEX = pdflatex
BIBTEX = bibtex
PDFTOPS = pdftops
AR = acroread
GV = gv
EV = evince
RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined"

PSFILE = GaugedScotoSeesaw-v2.ps 
PDFFILE = GaugedScotoSeesaw-v2.pdf

COPY = if test -r GaugedScotoSeesaw-v2.toc; then cp GaugedScotoSeesaw-v2.toc GaugedScotoSeesaw-v2.toc.bak; fi 
RM = /bin/rm -f


CLEAN=rm -f GaugedScotoSeesaw-v2.aux GaugedScotoSeesaw-v2.log GaugedScotoSeesaw-v2.dvi GaugedScotoSeesaw-v2.toc GaugedScotoSeesaw-v2.out GaugedScotoSeesaw-v2.blg GaugedScotoSeesaw-v2.mtc GaugedScotoSeesaw-v2.mtc1 GaugedScotoSeesaw-v2.rel GaugedScotoSeesaw-v2.vrb GaugedScotoSeesaw-v2.end GaugedScotoSeesaw-v2.spl GaugedScotoSeesaw-v2.synctex.gz GaugedScotoSeesaw-v2Notes.bib *~ \#* *.aux

WARNING=egrep -i "(Reference|Citation).*undefined" GaugedScotoSeesaw-v2.log ; true

HELP=cat /home/jv/bin/help/MakePDFLatexMakefile.help

main:	GaugedScotoSeesaw-v2.tex pdf

GaugedScotoSeesaw-v2.tex:	GaugedScotoSeesaw-sub.tex GaugedScotoSeesaw.tex
	touch GaugedScotoSeesaw-v2.tex

pdf:	$(PDFFILE)
	$(WARNING)  

all:	$(PDFFILE) $(PSFILE)
	$(WARNING)  

ps:	$(PSFILE) 
	$(WARNING)

gv:	$(PSFILE)
	$(GV) $(PSFILE) &
	$(WARNING)

	$(WARNING)

ev:	$(PDFFILE)
	$(EV) $(PDFFILE) &

ar:	$(PDFFILE)
	$(AR) $(PDFFILE) &

%.pdf:	%.tex
	$(COPY);$(LATEX) $<
	egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ;true
	egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
	egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
	if [  'cmp -s $*.toc $*.toc.bak'  ]; then $(LATEX) $< ; fi
	$(RM) $*.toc.bak

%.ps:	%.pdf
	$(PDFTOPS) $<

clean:	
	$(CLEAN)

realclean: 	
	$(CLEAN)
	$(RM) $(FILENAME).ps $(FILENAME).pdf $(FILENAME).bbl
	$(RM) $(FILENAME).lof $(FILENAME).lot $(FILENAME).rel

cleanps: 	
	$(CLEAN)
	$(RM) $(FILENAME).ps $(FILENAME).bbl

help:
	$(HELP)


